The Effects of Spatial Interpolation on a Novel, Dual-Doppler 3D Wind Retrieval Technique

Three-dimensional wind retrievals from ground-based Doppler radars have played an important role in meteorological research and nowcasting over the past four decades. However, in recent years, the proliferation of open-source software and increased demands from applications such as convective parameterizations in numerical weather prediction models has led to a renewed interest in these analyses. In this study, we analyze how a major, yet often-overlooked, error source effects the quality of retrieved 3D wind fields. Namely, we investigate the effects of spatial interpolation, and show how the common practice of pre-gridding radial velocity data can degrade the accuracy of the results. Alternatively, we show that assimilating radar data directly at their observation locations improves the retrieval of important dynamic features such as the rear flank downdraft and mesocyclone within a simulated supercell, while also reducing errors in vertical vorticity, horizontal divergence, and all three velocity components.

==> stats2.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab} Summary error statistics for the 15 member ensemble for each retrieval method. The ensemble mean and standard deviation (in parentheses) are shown for the total RMSE, RMSE within the analysis region (an.) and RMSE for individual wind components ($u$, $v$, $w$). Fractions Skill Scores (FSS) are also listed for updrafts (up, 95th percentile of the column maximum vertical winds) and downdrafts (down, 5th percentile of the column minimum vertical winds).}
\begin{tabular}{lrrrrrrr}
\toprule
{} &         RMSE &      RMSE an. &     RMSE $u$ &     RMSE $v$ &     RMSE $w$ &       FFS up &     FSS down \\
\midrule
Control     &  2.00 (0.05) &   2.68 (0.04) &  0.23 (0.13) &  0.22 (0.11) &  1.96 (0.03) &  0.95 (0.00) &  0.80 (0.02) \\
3D Cressman &  7.17 (0.16) &  11.61 (0.22) &  4.42 (0.28) &  4.25 (0.36) &  3.68 (0.16) &  0.70 (0.04) &  0.26 (0.04) \\
2D Cressman &  7.43 (0.37) &   8.90 (0.37) &  4.96 (0.45) &  4.28 (0.29) &  3.49 (0.14) &  0.76 (0.04) &  0.43 (0.05) \\
RA          &  6.22 (0.27) &   8.03 (0.61) &  3.77 (0.57) &  3.61 (0.52) &  3.30 (0.13) &  0.88 (0.01) &  0.63 (0.06) \\
\bottomrule
\end{tabular}
\end{table*}

